Characterising the secondary maximum in the r-band for Type Ia Supernovae: Diagnostic for the ejecta mass

An increase in the number of studied Type Ia supernovae (SNe~Ia) has demonstrated that this class of explosions has a greater diversity in its observables than was previously assumed. The reasons (e.g. the explosion mechanism, progenitor system) for such a diversity remain unknown. Here, we analyse a sample of $r$-band light curves of SNe~Ia, focusing on their behaviour $\sim$ 2-4 weeks after maximum light, i.e. the second maximum. We characterise the second maximum by its timing ($t_{r_2}$) and the integrated flux ($\overline{\mathcal{F}}_{r_2}$). We find that $t_{r_2}$ correlates with the "colour-stretch" parameter s$_{BV}$, which can be used as a proxy for $^{56}$Ni mass, and $\overline{\mathcal{F}}_{r_2}$, correlates with the transparency timescale, t$_0$. Using $\overline{\mathcal{F}}_{r_2}$, for a sample of 199 SNe from the Palomar Transient Factory and intermediate Palomar Transient Factory, we evaluate a distribution on t$_0$ for a sample of SNe~Ia found in an "untargeted" survey. Comparing this distribution to the predictions of t$_0$ ranges from models we find that the largest overlap in t$_0$ values between models and observations is for the sub-Chandrasekhar double detonation models. We also compare our relations between t$_0$ and $\overline{\mathcal{F}}_{r_2}$, with that from 1-D explosion models of \citet{GK18} and confirm that $\overline{\mathcal{F}}_{r_2}$, can be used as a diagnostic of the total ejecta mass.

==> ref.tex <==
\begin{thebibliography}{99}


\bibitem[\protect\citeauthoryear{Arnett}{1969}]{Arnett1969} Arnett W.~D., 1969, Ap\&SS, 5, 180 


\bibitem[\protect\citeauthoryear{Arnett}{1982}]{Arnett1982} Arnett 
W.~D., 1982, ApJ, 253, 785 

\bibitem[\protect\citeauthoryear{Arnett et al.}{1985}]{Arnett1985} Arnett 
W.~D., Branch D., Wheeler J. C., 1985, Nature, 314, 337


%\bibitem[\protect\citeauthoryear{Axelrod}{1980}]{Axelrod1980} 
%Axelrod T.~S., 1980, PhDT,  


%\bibitem[\protect\citeauthoryear{Barone-Nugent et 
%al.}{2012}]{Barone-Nugent2012} Barone-Nugent R.~L., et al., 2012, MNRAS, 
%425, 1007

%\bibitem[\protect\citeauthoryear{Benetti et 
%al.}{2004}]{Benetti2004} Benetti S., et al., 2004, MNRAS, 348, 261

\bibitem[\protect\citeauthoryear{M. Hicken et al.}{2009}]{Hicken2009} Hicken M., et al., 2009, ApJ, 700, 331H

\bibitem[\protect\citeauthoryear{Biscardi et 
al.}{2012}]{Biscardi2012} Biscardi I., et al., 2012, A\&A, 537, A57 

\bibitem[\protect\citeauthoryear{Blondin et 
al.}{2013}]{Blondin2013} Blondin S., Dessart L., Hillier D.~J., 
Khokhlov A.~M., 2013, MNRAS, 429, 2127 

\bibitem[\protect\citeauthoryear{Blondin, Dessart, 
\& Hillier}{2015}]{Blondin2015} Blondin S., Dessart L., Hillier D.~J., 2015, MNRAS, 448, 2766 


\bibitem[\protect\citeauthoryear{Branch}{1992}]{Branch1992} Branch 
D., 1992, ApJ, 392, 35
%\bibitem[\protect\citeauthoryear{Branch 
%\& Tammann}{1992}]{Branch1992} Branch D., Tammann G.~A., 1992, ARA\&A, 30, 359 
\bibitem[\protect\citeauthoryear{Burns et al.}{2011}]{Burns2011} 
Burns C.~R., et al., 2011, AJ, 141, 19 

\bibitem[\protect\citeauthoryear{Burns et al.}{2014}]{Burns2014} Burns
C.~R., et al., 2014, ApJ, 789, 32 

\bibitem[\protect\citeauthoryear{Cardelli, Clayton 
\& Mathis}{1989}]{Cardelli1989} Cardelli J.~A., Clayton G.~C.,
Mathis J.~S., 1989, ApJ, 345, 245 

\bibitem[\protect\citeauthoryear{Cartier et 
al.}{2014}]{Cartier2013} Cartier R., et al., 2014, ApJ, 789, 89

\bibitem[\protect\citeauthoryear{Chotard et 
al.}{2011}]{Chotard2011} Chotard N., et al., 2011, A\&A, 529, L4

\bibitem[\protect\citeauthoryear{Churazov et 
al.}{2014}]{Churazov2014} Churazov E., et al., 2014, Nature, 
512, 406
\bibitem[\protect\citeauthoryear{Churazov et 
al.}{2015}]{Churazov2015} Churazov E., et al., 2015, ApJ, 812, 62

%\bibitem[\protect\citeauthoryear{Colgate 
%\& McKee}{1969}]{Colgate1969} Colgate S.~A., McKee C., 1969, ApJ, 157, 623 


\bibitem[\protect\citeauthoryear{Contardo, Leibundgut 
\& Vacca}{2000}]{Contardo2000} Contardo G., Leibundgut B., Vacca W.~D., 2000, A\&A, 359, 876 

\bibitem[\protect\citeauthoryear{Contreras et 
al.}{2010}]{Contreras2010} Contreras C., et al., 2010, AJ, 139, 519 

\bibitem[\protect\citeauthoryear{Dado \& Dar}{2015}]{Dado2015} 
Dado S., Dar, A., 2015, ApJ, 809, 32

\bibitem[\protect\citeauthoryear{Dhawan et al.}{2015}]{Dhawan2015} 
Dhawan S., Leibundgut B., Spyromilio J., Maguire K., 2015, MNRAS, 448, 1345

\bibitem[\protect\citeauthoryear{Diehl et 
al.}{2015}]{Diehl2015} Diehl R., et al., 2015, A\&A, 574, A72 


%\bibitem[\protect\citeauthoryear{Diehl et al.}{2014}]{Diehl2014} 
%Diehl R., et al., 2014, Science, 345, 1162 
 

\bibitem[\protect\citeauthoryear{Elias-Rosa et
al.}{2006}]{ER06} Elias-Rosa N., et al., 2006, MNRAS, 369,
1880

\bibitem[\protect\citeauthoryear{Filippenko et
al.}{1992}]{Filippenko1992} Filippenko A.~V., et al., 1992, AJ, 104,
1543 

%\bibitem[\protect\citeauthoryear{Firth et al.}{2015}]{Firth2015} 
%Firth R.~E., et al., 2015, MNRAS, 446, 3895

%\bibitem[\protect\citeauthoryear{Folatelli et 
%al.}{2010}]{Folatelli2010} Folatelli G., et al., 2010, AJ, 139, 120 

%\bibitem[\protect\citeauthoryear{Foley et al.}{2014}]{2014MNRAS.443.2887F} 
%Foley R.~J., et al., 2014, MNRAS, 443, 2887 

%\bibitem[\protect\citeauthoryear{Foley et 
%al.}{2014}]{Foley2014} Foley R., et al., 2014, arXiv, 
%arXiv:1405.3677

%\bibitem[\protect\citeauthoryear{Foreman-Mackey et 
%al.}{2013}]{FM13} Foreman-Mackey D., Hogg D.~W., Lang D., 
%Goodman J., 2013, PASP, 125, 306
%\bibitem[\protect\citeauthoryear{Freedman et 
%al.}{2001}]{Freedman2001} Freedman W.~L., et al., 2001, ApJ, 553, 47 

\bibitem[\protect\citeauthoryear{Friedman et 
al.}{2015}]{Friedman2015} Friedman A.~S., et al., 2015, ApJS, 220, 9 

\bibitem[\protect\citeauthoryear{Ganeshalingam, Li, 
\& Filippenko}{2011}]{G11} Ganeshalingam M., Li W., Filippenko A.~V., 2011, MNRAS, 416, 2607 

\bibitem[\protect\citeauthoryear{Goldstein \& Kasen}{2018}] {GK18}Goldstein D. \& Kasen D., 2018, ApJ, 852, L33

\bibitem[\protect\citeauthoryear{Goobar}{2008}]{Goobar2008} Goobar 
A., 2008, ApJ, 686, L103 


%\bibitem[\protect\citeauthoryear{Goobar 
%\& Leibundgut}{2011}]{Goobar2011} Goobar A., Leibundgut B., 2011, ARNPS, 61, 251


\bibitem[\protect\citeauthoryear{Goobar et al.}{2014a}]{Goobar2014a} 
Goobar A., et al., 2014, ApJ, 784, L12 
\bibitem[\protect\citeauthoryear{Goobar et al.}{2015}]{Goobar2014b} 
Goobar A., et al., 2015, ApJ, 799, 106 
%\bibitem[\protect\citeauthoryear{Goobar et al.}{2014b}]{Goobar2014b} 
%Goobar A., et al., 2014, arXiv, arXiv:1410.1363  


%\bibitem[\protect\citeauthoryear{Go%odman \& Weare}{2010}]{Goodman2010} 
%Goodman J., Weare J., 2010, Comm. App. Math. Comp. Sci. 5 (1), 65.


\bibitem[\protect\citeauthoryear{Hachinger et 
al.}{2012}]{Hachinger2012} Hachinger S., Mazzali P.~A., Taubenberger 
S., Fink M., Pakmor R., Hillebrandt W., Seitenzahl I.~R., 2012, MNRAS, 427, 
2057 

\bibitem[\protect\citeauthoryear{Hillebrandt 
\& Niemeyer}{2000}]{Hillebrandt2000} Hillebrandt W., Niemeyer J.~C., 2000, ARA\&A, 38, 191 

%\bibitem[\protect\citeauthoryear{Hillebrandt {\ 
%R&ouml}pke}{2010}]{Hillebrandt2010} Hillebrandt W., R{\"o}pke F.~K., 2010, NewAR, 54, 201 


%\bibitem[\protect\citeauthoryear{Hillebrandt et 
%al.}{2013}]{Hillebrandt2013} Hillebrandt W., Kromer M., R{\"o}pke 
%F.~K., Ruiter A.~J., 2013, FrPhy, 8, 116 

%\bibitem[\protect\citeauthoryear{H\"oflich, Khokhlov \&
%Wheeler}{1995}]{Hoeflich1995} H\" oflich P., Khokhlov A., Wheeler C.,
%1995, ASPC, 73, 441 

%\bibitem[\protect\citeauthoryear{H{\"o}flich et 
%al.}{2010}]{Hoflich2010} H{\"o}flich P., et al., 2010, ApJ, 710, 
%444

%\bibitem[\protect\citeauthoryear{Jack, Hauschildt, 
%\& Baron}{2012}]{Jack2012} Jack D., Hauschildt P.~H., Baron E., 2012, A\&A, 538, A132 

%\bibitem[\protect\citeauthoryear{Jensen et
%al.}{2003}]{Jensen2003} Jensen J.~B., Tonry J.~L., Barris
%B.~J., Thompson R.~I., Liu M.~C., Rieke M.~J., Ajhar E.~A., Blakeslee
%J.~P., 2003, ApJ, 583, 712 

%\bibitem[\protect\citeauthoryear{Jha, Riess, 
%\& Kirshner}{2007}]{Jha2007} Jha S., Riess A.~G., Kirshner R.~P., 2007, ApJ, 659, 122 

\bibitem[\protect\citeauthoryear{Kasen}{2006}]{Kasen2006} Kasen 
D., 2006, ApJ, 649, 939

%\bibitem[\protect\citeauthoryear{Kasen 
%\& Woosley}{2007}]{Kasen2007} Kasen D., Woosley S.~E., 2007, ApJ, 656, 661 
 
%\bibitem[\protect\citeauthoryear{Kattner et al.}{2012}]{Kattner2012} Kattner S., et al., 2012, PASP, 124, 114 

%\bibitem[\protect\citeauthoryear{Katz, Kushnir, 
%\& Dong}{2013}]{Katz2013} Katz B., Kushnir D., Dong S., 2013, arXiv, arXiv:1301.6766 


%\bibitem[\protect\citeauthoryear{Kelly}{2007}]{Kelly2007} Kelly 
%B.~C., 2007, ApJ, 665, 1489 
%\bibitem[\protect\citeauthoryear{Krisciunas et 
%al.}{2001}]{K01} Krisciunas K., et al., 2001, AJ, 122, 1616 

%\bibitem[\protect\citeauthoryear{Krisciunas et 
%al.}{2003}]{K03} Krisciunas K., et al., 2003, AJ, 125, 166 
\bibitem[\protect\citeauthoryear{Khokhlov}{1991}]{Khokhlov1991} Khokhlov A.~M., 1991, A\&A, 245, 114 

%\bibitem[\protect\citeauthoryear{Khokhlov}{1993}]{Khokhlov1993} Khokhlov A.~M., 1993, A\&A, 270, 223

\bibitem[\protect\citeauthoryear{Khokhlov, Mueller, 
\& Hoeflich}{1993}]{Khokhlov1993} Khokhlov A., Mueller E., H\"oflich P., 1993, A\&A, 270, 223 

%\bibitem[\protect\citeauthoryear{Kozma et 
%al.}{2005}]{Kozma2005} Kozma C., Fransson C., Hillebrandt W., Travaglio C., Sollerman J., Reinecke M., R{\"o}pke F.~K., Spyromilio J., 2005, A\&A, 437, 983 



%\bibitem[\protect\citeauthoryear{Krisciunas et al.}{2004}]{Krisciunas2004} Krisciunas K., Phillips M.M., Suntzeff, N.B., 2004, ApJ, 602, 81

%\bibitem[\protect\citeauthoryear{Krisciunas et 
%al.}{2004}]{K04b} Krisciunas K., et al., 2004b, AJ, 127, 1664 

%\bibitem[\protect\citeauthoryear{Krisciunas et 
%al.}{2004}]{K04b} Krisciunas K., et al., 2004b, AJ, 128, 3034 

%\bibitem[\protect\citeauthoryear{Krisciunas et al.}{2007}]{Krisciunas2007} Krisciunas K., et al., 2007, AJ, 133, 58 

%\bibitem[\protect\citeauthoryear{Krisciunas et 
%al.}{2009}]{Krisciunas2009} Krisciunas K., et al., 2009, AJ, 138, 1584 

%\bibitem[\protect\citeauthoryear{Kromer 
%\& Sim}{2009}]{Kromer2009} Kromer M., Sim S.~A., 2009, MNRAS,
%398, 1809 

%\bibitem[\protect\citeauthoryear{Leaman et al.}{2011}]{Leaman2011} 
%Leaman J., Li W., Chornock R., Filippenko A.~V., 2011, MNRAS, 412, 1419 

%\bibitem[\protect\citeauthoryear{Leibundgut}{1988}]{Leibundgut1988} Leibundgut B., 1988, PhD thesis, University of Basel

%\bibitem[\protect\citeauthoryear{Leibundgut}{2000}]{Leibundgut2000} Leibundgut B., 2000, A\&ARv, 10, 179 

%\bibitem[\protect\citeauthoryear{Leibundgut}{2001}]{Leibundgut2001} Leibundgut B., 2001, ARA\&A, 39, 67 

\bibitem[\protect\citeauthoryear{Leibundgut et 
al.}{1993}]{Leibundgut1993} Leibundgut B., et al., 1993, AJ, 105,
301 

\bibitem[\protect\citeauthoryear{Leloudas et
al.}{2009}]{Leloudas2009} Leloudas G., et al., 2009, A\&A, 505, 265

%\bibitem[\protect\citeauthoryear{Leloudas et 
%al.}{2009}]{Leloudas2009} Leloudas G., et al., 2009, A\&A, 505, 265 

%\bibitem[\protect\citeauthoryear{Li et al.}{2001}]{Li2001} Li W., et
%al., 2001, PASP, 113, 1178 

%\bibitem[\protect\citeauthoryear{Li et al.}{2011}]{2011MNRAS.412.1441L} Li 
%W., et al., 2011, MNRAS, 412, 1441 %\bibitem[\protect\citeauthoryear{Li et al.}{2003}]{Li2003} Li W., et
%al., 2003, PASP, 115, 453 
\bibitem[\protect\citeauthoryear{Li et al.}{2011}]{Li2011} Li 
W., et al., 2011, MNRAS, 412, 1441 
%\bibitem[\protect\citeauthoryear{Lira}{1996}]{Lira1996} Lira P., 
%1996, MsT, 3 
\bibitem[\protect\citeauthoryear{Livio}{2000}]{Livio2000} Livio 
M., 2000, in: Type Ia Supernovae, Theory and Cosmology, ed. J. C. Niemeyer\& J. W. Truran, Cambridge: Cambridge University Press, 33 
%\bibitem[\protect\citeauthoryear{Maeda et al.}{2010}]{M10} 
%Maeda K., Taubenberger S., Sollerman J., Mazzali P.~A., Leloudas G., Nomoto 
%K., Motohara K., 2010, ApJ, 708, 1703 

%\bibitem[\protect\citeauthoryear{Maeda et al.}{2011}]{M11} 
%Maeda K., et al., 2011, MNRAS, 413, 3075 
%\bibitem[\protect\citeauthoryear{Maguire et 
%al.}{2012}]{Maguire2012} Maguire K., et al., 2012, MNRAS, 426, 2359 

%\bibitem[\protect\citeauthoryear{Marion et al.}{2009}]{Marion2009} 
%Marion G.~H., H{\"o}flich P., Gerardy C.~L., Vacca W.~D., Wheeler J.~C., 
%Robinson E.~L., 2009, AJ, 138, 727 

%\bibitem[\protect\citeauthoryear{Mandel et al.}{2009}]{Mandel2009} 
%Mandel K.~S., Wood-Vasey W.~M., Friedman A.~S., Kirshner R.~P., 2009, ApJ, 
%704, 629

\bibitem[\protect\citeauthoryear{Margutti et 
al.}{2014}]{Margutti2014} Margutti R., Parrent J., Kamble A., 
Soderberg A.~M., Foley R.~J., Milisavljevic D., Drout M.~R., Kirshner R., 
2014, ApJ, 790, 52

%\bibitem[\protect\citeauthoryear{Mazzali et 
%al.}{1997}]{Mazzali1997} Mazzali P.~A., Chugai N., Turatto M., Lucy 
%L.~B., Danziger I.~J., Cappellaro E., della Valle M., Benetti S., 1997, 
%MNRAS, 284, 151 

%\bibitem[\protect\citeauthoryear{Mazzali et 
%al.}{1998}]{Mazzali1998} Mazzali P.~A., Cappellaro E., Danziger 
%I.~J., Turatto M., Benetti S., 1998, ApJ, 499

\bibitem[\protect\citeauthoryear{Mazzali et 
al.}{2007}]{Mazzali2007} Mazzali P.~A., R{\"o}pke F.~K., Benetti 
S., Hillebrandt W., 2007, Science, 315, 825 

%\bibitem[\protect\citeauthoryear{Matheson et 
%al.}{2012}]{Matheson2012} Matheson T., et al., 2012, ApJ, 754, 19 

%\bibitem[\protect\citeauthoryear{Meikle}{2000}]{Meikle2000} Meikle 
%W.~P.~S., 2000, MNRAS, 314, 782 

\bibitem[\protect\citeauthoryear{Nadyozhin}{1994}]{Nadyozhin1994} 
Nadyozhin D.~K., 1994, ApJS, 92, 527 

%\bibitem[\protect\citeauthoryear{Nobili et 
%al.}{2005}]{Nobili2005} Nobili S., et al., 2005, A\&A, 437, 789 

%\bibitem[\protect\citeauthoryear{Nobili 
%\& Goobar}{2008}]{Nobili2008} Nobili S., Goobar A., 2008, A\&A, 487, 19 

%\bibitem[\protect\citeauthoryear{Pastorello et 
%al.}{2007}]{Pastorello2007} Pastorello A., et al., 2007, MNRAS, 377, 
%1531 

\bibitem[\protect\citeauthoryear{Nobili 
\& Goobar}{2008}]{Nobili2008} Nobili S., Goobar A., 2008, A\&A, 487, 19 

%\bibitem[Pankey(1962)]{Pankey1962}
%Pankey, T. 1962, Howard University Dissertation

%\bibitem[\protect\citeauthoryear{Pakmor et al.}{2012}]{Pakmor2012} 
%Pakmor R., Kromer M., Taubenberger S., Sim S.~A., R{\"o}pke F.~K., 
%Hillebrandt W., 2012, ApJ, 747, L10 

\bibitem[\protect\citeauthoryear{Patat et 
al.}{2013}]{Patat2013} Patat F., et al., 2013, A\&A, 549, A62 


\bibitem[\protect\citeauthoryear{Patat et 
al.}{2015}]{Patat2015} Patat F., et al., 2015, A\&A, 577, A53 



%\bibitem[\protect\citeauthoryear{Patat et al.}{2014}]{Patat2014} 
%Patat F., et al., 2014, arXiv, arXiv:1407.0136

\bibitem[\protect\citeauthoryear{Pereira et 
al.}{2013}]{Pereira2013} Pereira R., et al., 2013, A\&A, 554, A27 

%\bibitem[\protect\citeauthoryear{Perlmutter et
%al.}{1999}]{Perlmutter1999} Perlmutter S., et al., 1999, ApJ, 517, 565 

%\bibitem[\protect\citeauthoryear{Phillips}{1993}]{Phillips1993} 
%Phillips M.~M., 1993, ApJ, 413, L105 

\bibitem[\protect\citeauthoryear{Phillips}{2012}]{Phillips2012} 
Phillips M.~M., 2012, PASA, 29, 434 

\bibitem[\protect\citeauthoryear{Phillips et 
al.}{1987}]{Phillips1987} Phillips M.~M., et al., 1987, PASP, 99, 
592
%\bibitem[\protect\citeauthoryear{Phillips et 
%al.}{1999}]{Phillips1999} Phillips M.~M., Lira P., Suntzeff N.~B., 
%Schommer R.~A., Hamuy M., Maza J., 1999, AJ, 118, 1766 

%\bibitem[\protect\citeauthoryear{Phillips et 
%al.}{2006}]{Phillips2006} Phillips M.~M., et al., 2006, AJ, 131, 
%2615 

\bibitem[\protect\citeauthoryear{Phillips et 
al.}{2013}]{Phillips2013} Phillips M.~M., et al., 2013, ApJ, 779, 38 

\bibitem[\protect\citeauthoryear{Pignata et 
al.}{2008}]{Pignata2008} Pignata G., et al., 2008, MNRAS, 388, 971 

%\bibitem[\protect\citeauthoryear{Pinto 
%\& Eastman}{2000}]{Pinto2000} Pinto P.~A., Eastman R.~G., 2000, ApJ, 530, 757 

%\bibitem[\protect\citeauthoryear{Riess, Press, 
%\& Kirshner}{1996}]{Riess1996} Riess A.~G., Press W.~H., Kirshner R.~P., 1996, ApJ, 473, 88 




%\bibitem[\protect\citeauthoryear{Piro 
%\& Nakar}{2013}]{Piro2013} Piro A.~L., Nakar E., 2013, ApJ, 769, 6

%\bibitem[\protect\citeauthoryear{Piro 
%\& Nakar}{2014}]{Piro2014} Piro A.~L., Nakar E., 2014, ApJ, 784, 85 

%\bibitem[\protect\citeauthoryear{Riess et al.}{1998}]{Riess1998} 
%Riess A.~G., et al., 1998, AJ, 116, 1009 

%\bibitem[\protect\citeauthoryear{R{\"o}pke 
%\& Hillebrandt}{2004}]{Ropke2004} R{\"o}pke F.~K., Hillebrandt W., 2004, A\&A, 420, L1 


\bibitem[\protect\citeauthoryear{Ruiter et al.}{2013}]{Ruiter2013} 
Ruiter A.~J., et al., 2013, MNRAS, 429, 1425 

\bibitem[\protect\citeauthoryear{Ruiz-Lapuente 
\& Lucy}{1992}]{RL1992} Ruiz-Lapuente P., Lucy L.~B., 1992, ApJ, 400, 127 

%\bibitem[\protect\citeauthoryear{Scalzo et al.}{2010}]{Scalzo2010} 
%Scalzo R., et al., 2010, ApJ, 713, 1073 

%\bibitem[\protect\citeauthoryear{Scalzo et al.}{2012}]{Scalzo2012} 
%Scalzo R., et al., 2012, ApJ, 757, 12 

\bibitem[\protect\citeauthoryear{Scalzo et al.}{2010}]{Scalzo2010} 
Scalzo R.~A., et al., 2010, ApJ, 713, 1073 


%\bibitem[\protect\citeauthoryear{Scolnic et 
%al.}{2014}]{Scolnic2014} Scolnic D.~M., Riess A.~G., Foley R.~J., 
%Rest A., Rodney S.~A., Brout D.~J., Jones D.~O., 2014, ApJ, 780, 37 

\bibitem[\protect\citeauthoryear{Scalzo et al.}{2014}]{Scalzo2014} 
Scalzo R., et al., 2014, MNRAS, 440, 1498 

\bibitem[\protect\citeauthoryear{Sim et al.}{2010}]{Sim2010} 
Sim S.~A., R{\"o}pke F.~K., Hillebrandt W., Kromer M., Pakmor R., Fink M., 
Ruiter A.~J., Seitenzahl I.~R., 2010, ApJ, 714, L52 

%\bibitem[\protect\citeauthoryear{Sollerman et 
%al.}{2004}]{Sollerman2004} Sollerman J., et al., 2004, A\&A, 428, 555 


\bibitem[\protect\citeauthoryear{Stehle et al.}{2005}]{Stehle2005} 
Stehle M., Mazzali P.~A., Benetti S., Hillebrandt W., 2005, MNRAS, 360, 
1231 
  

\bibitem[\protect\citeauthoryear{Stritzinger et 
al.}{2006}]{Stritzinger2006b} Stritzinger M., Mazzali P.~A., Sollerman J., Benetti S., 2006, A\&A, 460, 793 



\bibitem[\protect\citeauthoryear{Stritzinger et 
al.}{2011}]{Stritzinger2011} Stritzinger M.~D., et al., 2011, AJ, 142, 
156 
\bibitem[\protect\citeauthoryear{Suntzeff}{1996}]{Suntzeff1996} 
Suntzeff N.~B., 1996, in: Supernovae and supernova remnants, ed. Richard McCray \& Zhenru Wang, Cambridge: Cambridge University Press, 41 

\bibitem[Suntzeff(2003)]{Suntzeff2003} 
Suntzeff, N.~B. 2003, in: From Twilight to Highlight, The Physics of 
Supernovae, ed. W. Hillebrandt \& B. Leibundgut, Heidelberg:Springer, 
183 

\bibitem[\protect\citeauthoryear{Taubenberger et 
al.}{2011}]{T11} Taubenberger S., et al., 2011, MNRAS, 412, 
2735 

\bibitem[\protect\citeauthoryear{Taubenberger et 
al.}{2013}]{T13} Taubenberger S., et al., 2013, MNRAS, 432, 
3117 


%\bibitem[\protect\citeauthoryear{Tonry et al.}{2001}]{Tonry2001} 
%Tonry J.~L., Dressler A., Blakeslee J.~P., Ajhar E.~A., Fletcher A.~B., 
%Luppino G.~A., Metzger M.~R., Moore C.~B., 2001, ApJ, 546, 681

\bibitem[\protect\citeauthoryear{Travaglio et 
al.}{2004}]{Travaglio2004} Travaglio C., Hillebrandt W., Reinecke M., Thielemann F.-K., 2004, A\&A, 425, 1029 


%\bibitem[\protect\citeauthoryear{Tripp}{1998}]{Tripp1998} Tripp R., 1998, A\&A, 331, 815 

\bibitem[\protect\citeauthoryear{Truran, Glasner, 
\& Kim}{2012}]{Truran2012} Truran J.~W., Glasner A.~S., Kim Y., 2012, JPhCS, 337, 012040 
%\bibitem[\protect\citeauthoryear{Tully}{1988}]{Tully1988} Tully 
%R.~B., 1988, ngc..book,
%\bibitem[\protect\citeauthoryear{Valentini et 
%al.}{2003}]{Valentini2003} Valentini G., et al., 2003, ApJ, 595,
%779 
\bibitem[\protect\citeauthoryear{van Kerkwijk, Chang, 
\& Justham}{2010}]{VK2010} van Kerkwijk M.~H., Chang P., Justham S., 2010, ApJ, 722, L157 


%\bibitem[\protect\citeauthoryear{Wang et al.}{2008}]{Wang} 
%Wang B., Meng X.-C., Wang X.-F., Han Z.-W., 2008, ChJAA, 8, 71

\bibitem[\protect\citeauthoryear{Wang et al.}{2008}]{Wang2008} 
Wang X., et al., 2008, ApJ, 675, 626 

%\bibitem[\protect\citeauthoryear{Wood-Vasey et 
%al.}{2008}]{Wood-Vasey2008} Wood-Vasey W.~M., et al., 2008, ApJ, 689, 
%377 

%\bibitem[\protect\citeauthoryear{Weyant et al.}{2014}]{Weyant2014} 
%Weyant A., Wood-Vasey W.~M., Allen L., Garnavich P.~M., Jha S.~W., Joyce 
%R., Matheson T., 2014, ApJ, 784, 105 

\bibitem[\protect\citeauthoryear{Woosley}{1990}]{Woosley1990} 
Woosley S.~E., 1990, BAAS, 22, 1221 
 

\bibitem[\protect\citeauthoryear{Woosley 
\& Weaver}{1994}]{WW94} Woosley S.~E., Weaver T.~A., 1994, ApJ, 423, 371 

%\bibitem[\protect\citeauthoryear{Zheng et al.}{2014}]{Zheng2014} 
%Zheng W., et al., 2014, ApJ, 783, LL24 

\end{thebibliography}
